ReTabAD: A Benchmark for Restoring Semantic Context in Tabular Anomaly Detection

In tabular anomaly detection (AD), textual semantics often carry critical signals, as the definition of an anomaly is closely tied to domain-specific context. However, existing benchmarks provide only raw data points without semantic context, overlooking rich textual metadata such as feature descriptions and domain knowledge that experts rely on in practice. This limitation restricts research flexibility and prevents models from fully leveraging domain knowledge for detection. ReTabAD addresses this gap by restoring textual semantics to enable context-aware tabular AD research. We provide (1) 20 carefully curated tabular datasets enriched with structured textual metadata, together with implementations of state-of-the-art AD algorithms including classical, deep learning, and LLM-based approaches, and (2) a zero-shot LLM framework that leverages semantic context without task-specific training, establishing a strong baseline for future research. Furthermore, this work provides insights into the role and utility of textual metadata in AD through experiments and analysis. Results show that semantic context improves detection performance and enhances interpretability by supporting domain-aware reasoning. These findings establish ReTabAD as a benchmark for systematic exploration of context-aware AD.

==> figures/ablation.tex <==
\begin{wrapfigure}{r}{0.55\textwidth}
  \centering
  \vspace{-5mm} % 텍스트와의 간격 조정
  \includegraphics[width=1\linewidth]{figures/main_figure/missing.pdf}
  \caption{\textbf{AUROC Performance Change under Noisy and Corrupted data.} 
  (i.e., Gaussian noise, missing value, feature swap). 
  X-axis denotes severity. 
  Y-axis denotes the \% of performance change (macro-averaged $\Delta$AUROC).}
  \label{fig:robust}
  \vspace{-3mm} % 캡션 후 여백
\end{wrapfigure}
% \begin{figure}[t]
%   \centering
%   \includegraphics[width=1\linewidth]{figures/main_figure/missing.pdf}
%   \caption{\textbf{AUROC Performance Change under Noisy and Corrupted data.} (i.e., Gaussian noise, missing value, feature swap). X-axis denotes severity. Y-axis denotes the \% of performance change (macro-averaged $\Delta$AUROC), and its range remains consistent across different algorithms.}
% \label{fig:robust}
% \end{figure}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.8\linewidth]{figures/main_figure/type_ablation.pdf}
%   \caption{
%   \textbf{Win rate comparison across different context types on the \bmname benchmark.}}

% \end{figure}


==> figures/main_result.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.8\linewidth]{figures/main_figure/auroc_boxplot_colored.pdf}
  \caption{
  \textbf{\textbf{AUROC Performance on the \bmname.}
This figure compares training-based methods and zero-shot LLMs (Gemini-2.5-pro, Best performing LLM).
LLMs with textual metadata consistently outperform the \textit{No Description} setting, confirming the importance of semantic context.
The LLM-based method with full descriptions reaches performance comparable to state-of-the-art baselines.
Hyperparameters for training-based methods are faithfully searched, and full results with detailed settings are provided in the appendix.}
% \bmname follows two guiding principles in data collection and annotation.
% (1) It preserves \textit{semantically-rich table data} by retaining original numerical and categorical values without transformations that distort semantics (e.g., one-hot encoding, text embedding).
% (2) It provides \textit{structured textual metadata} that specifies domains, feature characteristics, and normality criteria.
% Together, these principles enable evaluation of anomaly detection methods that exploit both numerical patterns and semantic context, laying the foundation for semantic-aware anomaly detection.
  }
  \label{fig:main_box}
\end{figure}

